An algorithm for computing the $\Upsilon$-invariant and the $d$-invariants of Dehn surgeries

By using grid homology theory, we give an explicit algorithm for computing Ozsv\'ath-Stipsicz-Szab\'o's $\Upsilon$-invariant and the $d$-invariant of Dehn surgeries along knots in $S^3$. As its application, we compute the two invariants for all prime knots with up to 11 crossings.

==> 8.tex <==
\section{Glossary of notation}
\label{sec: glossary}

We give a quick glossary of notation by section number:

\noindent
\begin{multicols}{2}
\begin{list}{}{}
\item[$C_n$] the degree $n$ complex of $C$, \ref{poset filtered chain complexes}.
\item[$C_R$] the subcomplex of $C$ associated to $R$, \ref{poset filtered chain complexes}.
\item[$C^r$] the reflection of $C$, \ref{poset filtered chain complexes}.
\item[$\mC$] the knot concordance group, ***.
\item[$\mC_{\np}$] the set of $\np$-equivalence classes of knots, \ref{np equivalence}.
\item[$CFK^{\infty}$] Heegaard Floer knot complex over $\F[U^{\pm 1}]$, \ref{subsubsec: CFK}.
\item[$CFK^-$] Heegaard Floer knot complex over $\F[U]$
\item[$cl(S)$] the closure of $S$, \ref{subsec: computing G_0(K^*) from G_0(K)}.
\item[$\CR(P)$] the set of closed regions of $P$, \ref{poset filtered chain complexes}.
\item[$\CR^{ss}(\Z^2)$] the set of semi-simple regions of $\Z^2$, \ref{subsec: computing G_0(K^*) from G_0(K)}.
\item[$d$] Ozsv\'ath-Szab\'o's $d$-invariant
\item[$\partial$] boundary map, \ref{poset filtered chain complexes}.
\item[$\F$] the field of order $2$, \ref{poset filtered chain complexes}.
\item[$\mF_i$] $\Z$-filtration, \ref{poset filtered chain complexes}.
\item[$\G_0$] the invariant $\G_0$, \ref{the invariant G_0}.
\item[$\tG_0$] the invariant $\tG_0$, \ref{the invariant G_0}.
\item[$\G_0^{(n)}$] the invariant $\G_0^{(n)}$, \ref{generalization of G_0}.
\item[$\tG^{(n)}_0$] the invariant $\tG_0^{(n)}$, \ref{generalization of G_0}.
\item[$\gen_0(C;R)$] the set of realizers of $R$ in $C$, \ref{tG_0 and G_0}.
\item[$\gr$] the homological grading, ***.
\item[$H_*(C)$] the homology group of $C$, \ref{poset filtered chain complexes}.
\item[$H_n(C)$] the degree $n$ homology group of $C$, \ref{poset filtered chain complexes}.
\item[$K$] a knot
\item[$-K$] the inverse of $K$
\item[$K^*$] the mirror image of $K$
\item[$\Lambda$] the ring $\F[U^{\pm 1}]$, \ref{subsubsec: CFK}.
\item[$\np$] Hom-Wu's $\np$-invariant
\item[$\nuplus$] $\np$-equivalence, \ref{np equivalence}.
\item[$P$] a poset, \ref{poset filtered chain complexes}.
\item[$\mathcal{P}(\CR(\Z^2))$] the power set of $\CR(\Z^2)$, \ref{the invariant G_0}.
\item[$\heq{P}{\sR}$] $P$-filtered homotopy equivalence over $\sR$, \ref{poset filtered chain complexes}.
\item[$R$] a closed region, \ref{poset filtered chain complexes}.
\item[$S$] a subset of $\Z^2$, \ref{subsec: computing G_0(K^*) from G_0(K)}. 
\item[$\mathcal{S}$] a subset of $\CR(\Z^2)$, \ref{the invariant G_0}.
\item[$S^3_{p/q}(K)$] the $p/q$-surgery along $K$
\item[$\tau$] Ozsv\'ath-Szab\'o's $\tau$-invariant
\item[$\Upsilon$] Ozsv\'ath-Stipsicz-Szab\'o's $\Upsilon$-invariant
\item[$V_k$] Ni-Wu's $V_k$ sequence

\end{list}
\end{multicols}
